Decongestion by Representation: Learning to Improve Economic Welfare in Marketplaces

Congestion is a common failure mode of markets, where consumers compete inefficiently on the same subset of goods (e.g., chasing the same small set of properties on a vacation rental platform). The typical economic story is that prices decongest by balancing supply and demand. But in modern online marketplaces, prices are typically set in a decentralized way by sellers, and the information about items is inevitably partial. The power of a platform is limited to controlling representations -- the subset of information about items presented by default to users. This motivates the present study of decongestion by representation, where a platform seeks to learn representations that reduce congestion and thus improve social welfare. The technical challenge is twofold: relying only on revealed preferences from the choices of consumers, rather than true preferences; and the combinatorial problem associated with representations that determine the features to reveal in the default view. We tackle both challenges by proposing a differentiable proxy of welfare that can be trained end-to-end on consumer choice data. We develop sufficient conditions for when decongestion promotes welfare, and present the results of extensive experiments on both synthetic and real data that demonstrate the utility of our approach.

==> analysis1.tex <==
\section{\blue{On Congestion and Welfare}}

\todo{decide what goes in and how:\\
- perceived prices \\
- david's new theory \\
- monotonicity \\
other?
}

\paragraph{Interpretation.}
\todo{where to plug this paragraph? maybe `good proxy' section?}
In our setting, the system cannot set prices directly.
However, we argue that representations provide a similar means for optimizing welfare.
Rewrite perceived value as:
\todo{redefine perceived values in term of utility/profit, so that $\pval - p = v - \ptilde$, and $\ptilde \ge p$}
\begin{equation}
\label{eq:reps_as_indiv_prices}
\pval_i(z_j) = 
v_i(x_j) + \pval_i(z_j) - v_i(x_j) =
v_i(x_j) - \beta_i^\top ((1-\mu) \odot x_j) = 
v_i(x_j) - \ptilde_{ij}
\end{equation}
Here, $\ptilde_{ij}$ are \emph{individualized pseudo-prices},
derived from information regarding $x_j$ missing in $z_j$.
Perceived values $\pval_{i}$---on which users act---can therefore be thought of as true values minus pseudo-prices (instead of true prices).
In this sense setting representations in effect sets `prices'.
Note that since pseudo-prices are individualized, they are more expressive than conventional (anonymous) prices,
but are also constrained by the structure of representations, and so cannot take arbitrary values.

\todo{perhaps talk about need for non-anonymous (perceived) prices, ie, anonymous can't get the job done under partial info. partial info inherently adds variation in how users perceive value, so the only way to correct for this is individualized prices (??)}

\todo{maybe connect to Hayek theory of prices as info; talk about indiv prices as multi-dim (vs uni-dim of anon prices)}



%----------------------------------------------------------------------

\blue{
\subsection{Monotonicity}
}

The core of our approach relies on minimizing congestion as a proxy for maximizing welfare.
% At the core of our approach lies the idea that minimizing congestion can be a useful proxy for maximizing welfare.
It is therefore natural to ask: when does decongestion improve welfare?
Focusing on individual markets,
in this section %we give sufficient conditions that guarantee \emph{monotonicity},
we study the conditions under which a market has the property of monotonicity, 
i.e., that welfare increases as congestion decreases.
We propose several definitions of monotonicity, and discuss policy implications. \looseness=-1
For the formal discussion we will define congestion in terms of the number of allocated items, as $n - \text{\# allocated items}$. Note that this is equivalent in our setting to a definition in terms of choices.\footnote{Equivalently, one can write the congestion in terms of choices as the total number of over-congested choices plus the total number of null choices, as follows, $\sum_j\max(0,(\sum_i y_{ij}) - 1) + \sum_i y_{i0}$. 
That is, the congestion increases with the number of over-congested chosen items and with the number of null choices.} 

%\subsection{Ex-post monotonicity}
Our first definition of montonicity is highly general:
it considers only welfare and congestion,
and therefore abstracts away all other elements of our setting
(choices, features, masks, perceived values, prices, tie-breaking (e.g., non-random), etc.). For this reason, it is also the most demanding.
% Let $m$ be some market with $n'$ users and $n$ items and valuations $v_{ij}$.
%, and denote valuations $V$ as $V_{ij} = v_i(x_j)$.
% We will operationally define congestion $c$ as $n$ minus the number of allocated items,
% i.e., $c=n-\sum_{ij} a_{ij}$.
\gn{Change notations? n for number of users, m for number of items, and we can use M to denote a market.}
\begin{definition} \label{def:expost} A market $M$ with valuations $v_{ij}$ is \emph{ex-post monotone} 
if for all $r \in [m]$,
any allocation of $r$ items gives (weakly) better welfare than any allocation of $t < r$  items.
\end{definition}
Simply put, ex-post monotone markets are those in which it is always better to allocate more items---irrespective of which items, and to which users.
Operationally, 
% if we define congestion as the total number minus the number of allocated items, then
less items will be allocated if there is more congestion---hence, ex-post monotone markets fair better under decongested choice profiles.
Note this property depends only on the $v_{ij}$, and is agnostic to any other properties of the market.

Not all markets are ex-post monotone:
% Note that such monotonicity does not hold in general.
For example, consider a market with two items and two users, %$n=n'=2$,
with $v_{11}=5$ and $v_{12}=2$ for User 1,
and $v_{21}=2$ and $v_{22}=1$ for User 2.
For $r=2$ allocated items, a decongested allocation of
item 2 to User 1 and item 1 to User 2 
% there is an allocation (obtained from a decongested choice profile) that
results in a welfare of 4;
however, for $r=1$, a congested allocation in which item 1 is given to User 1 
obtains a higher welfare of 5.

Given this, our next result gives a simple sufficient condition for ex-post monotonicity.
\begin{proposition}
\label{prop:ex_post_monotone}
Let $m$ be a market of $n$ items and $n'$ users with valuations $v_{ij}$.
Denote $\vmin = \min_{ij} v_{ij}$ and $\vmax = \max_{ij} v_{ij}$.
If $\vmax - \vmin \le \vmin / (n-1)$, then $m$ is ex-post monotone. 
\end{proposition}
\todo{consider restating as $\frac{\vmin}{\vmax} \ge \frac{n-1}{n}$; how does cor. apply then?}
Proof in Appendix \toref.
Intuitively, Prop. \ref{prop:ex_post_monotone} states that
when the \emph{range} of values (LHS) is sufficiently small
relative to the general \emph{scale} of values, normalized by the market size (RHS),
then congested choice profiles are always less efficient than decongested choice profiles.
This implies that even for the lowest-valued item in $m$,
whether it is allocated or not is significant in terms of welfare.
Note that a tighter condition can be obtained directly from the definition, but requires calculating optimal allocations, which is computationally hard (see Appendix XX for formal details). 

\begin{comment}
% \paragraph{Monotonizing markets.}
Prop.~\ref{prop:ex_post_monotone} also provides a simple recipe for \emph{monotonizing} markets:
% \emph{made} to be monotone.
\begin{corollary}
\label{cor:monotonize}
For any non-monotone market $m$,
there is a constant $b$ such that adding $b$ to all $v_{ij}$
makes $m$ monotone.
\end{corollary}
This holds since adding $b$ increases $\vmin$ (RHS), but does not affect $\vmax-\vmin$ (LHS).
Thus, if values are generally (and uniformly) increased, then decongestion becomes more effective as a proxy for welfare.
Conversely, a market can also be monotonized by uniformly decreasing prices
(as long as $p \ge 0$ is preserved).
More generally, Corr.~\ref{cor:monotonize} suggests that higher values---or lower prices---are better; hence, when multiple eqbuilibium prices $p^*$ exist,
we can expect lower prices to entail more monotonicity.\looseness=-1
\end{comment}

When we consider a market and whether it is worthwile to reduce congestion in that market, then on the one hand, if Def. \ref{def:expost} holds it provides us with very strong guarantees: monotonicity will be sustained under any user behavior and any allocation rule. However, on the other hand, this property might break for some markets due to allocation profiles that are not feasible in the market. The following definition of monotonicity still considers ex-post outcomes, but limits its scope to the setting of the given market.   


\begin{definition} Given a choice rule $c$, an allocation rule $a$, and a mask size $k$, a market $(users, items, prices)$ is called 
%\emph{Ex-Post Welfare Monotone in Congestion w.r.t. k-masked choices} 
\emph{Ex-Post Monotone w.r.t. $(c,a,k)$} 
if every feasible allocation of $s \in [m]$ items has at least the same welfare as every feasible allocation of $t < s$ items. %An allocation is called feasible if there exists a $k$-mask that induces user choices such that there exists a mapping under the allocation rule $a$. 
A feasible allocation is an allocation that can be obtained under the allocation rule $a$ from the choices induced according to $c$ by some $k$-mask.
\end{definition}

Lastly, there are scenarios where ex-post definitions of monotonicity are too strict, as they may break due to low probability events, or in cases that have a small impact on welfare. The following definition describes scenarios in which reducing congestion will increase welfare in expectation, rather than in every possible scenario.  

\begin{definition} Given a choice rule $c$, an allocation rule $a$, and a mask size $k$, a market $(users, items, prices)$ is called 
%\emph{Ex-Ante Welfare Monotone in Congestion w.r.t. k-masked choices}
\emph{Ex-Ante Monotone} %w.r.t. k-Masked Choices} 
w.r.t. $(c,a,k)$ 
if for every $k$-mask under which in expectation $s \leq m$ items are chosen  according to $c$, the expected welfare is at least the same as the expected welfare of every $k$-mask under which in expectation $t < s$ items are chosen according to $c$. (The expectation is over $c$ and $a$.)
\end{definition}

Notice that the above definitions are ordered according to their generality: Definition \ref{def:expost} implies Definitions \ref{def:market-ex-post} and \ref{}, and Definition \ref implies Definition \ref{}.
In Section \ref{} we explore the extent to which the above notions of motonicity hold in real data and show that ... \todo{}

% Empirical analysis:
In the next section we evaluate our learning approach on data from Movielens. In this dataset, we found that X\% of the markets are ex-post monotone. When considering the second and third notions of monotonicity, Figure XX shows the percentage of markets that are monotone as a function of the mask size $k$, and shows that \todo{...}. This empirical analysis shows that decreasing congestion indeed connects to improving welfare and motivates our approach. 
\begin{itemize}
    \item What percentage of markets in our data are ex-post monotone?
    \item What percentage are market ex-post monotone?
    \item What percentage are ex-ante monotone?
    \item Distribution of some distance of markets from monotonicity. E.g., perhaps monotonicity up to $l$ items (i.e., for $l=1$, there exist a single item that if we exclude it from the market it becomes monotone; thus the market is generally monotone but there are $l$ ``problematic'' items. Then, we can show the percentage of monotone markets as a function $l$.). 
    
\end{itemize}



\red{
as certificates:
- when can we compute? what do we need to observe?
[- post-hoc? assuming users report $v$ after the fact; can we work with $v_{i},y_i$, or do we need all $v_{ij}$-s?]
[- approximate?]
}


% \begin{definition} Given a choice rule $c$, an allocation rule $a$, and a mask size $k$, a market $(users, items, prices)$ is called 
% %\emph{Ex-Post Welfare Monotone in Congestion w.r.t. k-masked choices} 
% \emph{Ex-Post Monotone w.r.t. $(c,a,k)$} 
% if every feasible allocation of $s \leq m$ items has at least the same welfare as every feasible allocation of $t < s$ items. %An allocation is called feasible if there exists a $k$-mask that induces user choices such that there exists a mapping under the allocation rule $a$. 
% A feasible allocation is an allocation that can be obtained under the allocation rule $a$ from the choices induced according to $c$ by some $k$-mask.
% \end{definition}

% \begin{definition} Given a choice rule $c$, an allocation rule $a$, and a mask size $k$, a market $(users, items, prices)$ is called 
% %\emph{Ex-Ante Welfare Monotone in Congestion w.r.t. k-masked choices}
% \emph{Ex-Ante Monotone} %w.r.t. k-Masked Choices} 
% if for every $k$-mask under which in expectation $s \leq m$ items are chosen  according to $c$, the expected welfare is at least the same as the expected welfare of every $k$-mask under which in expectation $t < s$ items are chosen according to $c$. (The expectation is over $c$ and $a$.)
% \end{definition}
    

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

